Techtile: a Flexible Testbed for Distributed Acoustic Indoor Positioning and Sensing

The proposed infrastructure, named Techtile, provides a unique R&D facility as features dispersed electronics enables transmission and capturing of a multitude of signals in 3D. Specific available equipment that enhances the design process from smooth prototyping to a commercial product is discussed. The acoustic parameters of the room, particularly the reverberation and ambient noise, are measured to take these into account for future innovative acoustic indoor positioning and sensing systems. This can have a positive influence on the accuracy and precision. The wooden construction represents an acoustically challenging room for audible sound with a maximum measured RT60 value of 1.17s at 5kHz, which is comparable to the reverberation properties of a lecture or small concert hall. For ultrasound it is rather challenging due to the present ambient noise sources. In general, the Techtile room can be compared with a home or quiet office environment, in terms of sound pressure levels (SPLs). In addition to the acoustic properties, possible research and development options are discussed in combination with the associated challenges. Many of the designs described are available through open source.

==> tikz/mic_schematic.tex <==
% \documentclass{minimal}
% \usepackage{tikz}
% \usetikzlibrary{shapes,arrows}
% \usetikzlibrary{shapes.multipart}
% \usetikzlibrary{arrows.meta}
% \usepackage[europeanresistors,americaninductors]{circuitikz}
% \usetikzlibrary{patterns}
% \begin{document}

\begin{tikzpicture}[circuit ee IEC, american voltages, every text node part/.style={align=center}, /tikz/circuitikz/tripoles/nigfetd/height=.8, /tikz/circuitikz/tripoles/nigfetd/width=.5, small circuit symbols]

% sizes
\ctikzset{bipoles/resistor/height=0.15}
\ctikzset{bipoles/resistor/width=0.4}
\ctikzset{bipoles/capacitor/height=0.4}
\ctikzset{bipoles/capacitor/width=0.1}
\ctikzset{bipoles/americaninductor/height=0.35}
\ctikzset{bipoles/americaninductor/width=0.8}

\tikzset{block/.style = {rectangle, draw=black, thick, minimum width=1.5cm, minimum height = 2cm}}


\draw[color=white]
(-1,0) -- (8,0)
;


% create nodes
\node[op amp, yscale=-1, xscale=1](opamp) at (6, 0) {};
\node[op amp, yscale=-1, xscale=1](opamp) at (11, -0.50) {};
% microphone
\node [block] at (0,0) () {};

% \draw[color=black!80]
% (-1,1) to[sinusoidal voltage source, /tikz/circuitikz/bipoles/length=30pt] node [right, shift={(0cm,0.15cm)}] {$V_S cos(\omega t)$} (-1,-1)
% (-1,1) to[L, l_=$L_P$] (3, 1)
% (5,1) -- (8,1) to [R, /tikz/circuitikz/bipoles/length=50pt, l=$R_L$](8,-1)
% ;


% \ctikzset{bipoles/thickness=6}
% \ctikzset{bipoles/capacitor/height=0.5}
% \ctikzset{bipoles/capacitor/width=0.2}
% \draw[color=black!80]
% (3,1)  to[C, l_=$C_A$] (4,1) -- (5,1)
% (-1,-1) -- (2,-1) to[C, l=$C_B$] (5,-1)
% (5,-1) -- (8,-1);


\draw
% Create names or text
% mic
(0, 1.4) node[rectangle](r){IMP23ABSU}
(0.30, 0) node[rectangle](out){OUT}
(-0.3, 0.60) node[rectangle](vdd_mic){VDD}
(-0.3, -0.60) node[rectangle](gnd_mic){GND}

% C on VDD and GND mic
(-0.75, 0.60) -- (-1.3,0.60) to[C] node[shift={(0.3cm, 0.65cm)}]{$C_2$} (-1.3,-0.6) -- (-0.75,-0.6)
(-1.2,0.60) -- (-2.2,0.6) to [C] node[shift={(0.25cm, 0.65cm)}]{$C_1$} (-2.2,-0.6) -- (-1.2,-0.6)
(-2.2,0.6) to [short,-o] (-2.2,1) coordinate (1_8Vmic)
(-2.2, 1.4) node[rectangle](1_8V){1.8V}
(-2.2,-0.6) to (-2.2,-1) coordinate (a1)
node[ground, rotate=-90] at (-2.2,-1.1) {}

% Between mic and first OPAMP
(0.75, 0) -- (2,0)

%(0, 0.6) to [R, /tikz/circuitikz/bipoles/length=50pt, l=$R_L$](8,0.6)
%(opamp.+) to[short, -o]++(-1,0) coordinate (in)
%(micr) to [short, opamp.+] ++ (-1,0) coordinate (in)




\end{tikzpicture}
% \end{document}
